Evolving Collaboration, Dependencies, and Use in the Rust Open Source Software Ecosystem

Open-source software (OSS) is widely spread in industry, research, and government. OSS represents an effective development model because it harnesses the decentralized efforts of many developers in a way that scales. As OSS developers work independently on interdependent modules, they create a larger cohesive whole in the form of an ecosystem, leaving traces of their contributions and collaborations. Data harvested from these traces enable the study of large-scale decentralized collaborative work. We present curated data on the activity of tens of thousands of developers in the Rust ecosystem and the evolving dependencies between their libraries. The data covers seven years of developer contributions to Rust libraries and can be used to reconstruct the ecosystem's development history, such as growing developer collaboration networks or dependency networks. These are complemented by statistics on downloads and popularity, tracking the dynamics of use and success over time. Altogether the data give a comprehensive view of several dimensions of the ecosystem.

==> inputs/tables_description.tex <==
%\toprule
%\hline
\setlength\tabcolsep{2.5pt}
Table Name & Description\\
%\midrule
\hline
\verb+commit_comment_reactions+ & Individual emoji reactions to commit comments \\
\verb+commit_comments+ &  Comments to commits \\
\verb+commit_parents+ & Parenthood relationships between commits. Typically one per commit, can be 0 or more. \\
\verb+commit_repos+ & Repos to which commits belong. Min. one, can be several via forks. \\
\verb+commits+ & Listing metadata about specific commits \\
\verb+filtered_deps_package+ & Packages wich are filtered when appearing as a dependency to avoid cycles \\
\verb+filtered_deps_packageedges+ & Dependency edges between packages filtered to avoid cycles \\
\verb+filtered_deps_repo+ & Repositories wich are filtered when appearing as a dependency to avoid cycles \\
\verb+filtered_deps_repoedges+ & Edges directly discarded in the dependency graph \\
\verb+followers+ & Listing followers of GitHub accounts \\
\verb+forks+ & Listing forks declared on GitHub \\
\verb+identities+ & Listing each individual identity of the developers (email, GitHub account, Gitlab account) \\
\verb+identity_types+ & Listing of identitiy types (email, GitHub account, Gitlab account) \\
\verb+issue_comment_reactions+ & Individual emoji reactions to issue comments \\
\verb+issue_comments+ & Comments to issues \\
\verb+issue_labels+ & Individual labels of each issue \\
\verb+issue_reactions+ & Individual emoji reactions to each issue \\
\verb+issues+ & Listing of issues per repository \\
\verb+merged_identities+ & Keeping track of identities having been merged, for information purposes \\
\verb+merged_repositories+ & Repositories having been merged (after identifying renaming or typo in URL) \\
\verb+org_memberships+ & Membership of organization declared on GitHub for GitHub users. \\
\verb+organizations+ & Organizations or work groups as declared on GitHub \\
\verb+package_dependencies+ & Listing package dependencies (version to package with semver) \\
\verb+package_version_downloads+ & Listing daily downloads of package versions \\
\verb+package_versions+ & Listing versions of packages \\
\verb+packages+ & Listing packages \\
\verb+pullrequest_comment_reactions+ & Individual emoji reactions to each pull request \\
\verb+pullrequest_comments+ & Comments to each pull request \\
\verb+pullrequest_labels+ & Individual labels of each pull request \\
\verb+pullrequest_reactions+ & Individual emoji reactions to each pull request \\
\verb+pullrequests+ & Listing of pull requests per repository \\
\verb+repo_languages+ & Listing language composition of repositories (GitHub) \\
\verb+repositories+ & Listing repositories \\
\verb+sources+ & Listing data sources \\
\verb+sponsors_user+ & Listing sponsorships of developers \\
\verb+stars+ & Listing starring events of repositories \\
\verb+urls+ & Listing retrieved URLs, and their parsed equivalent \\
\verb+user_languages+ & Language composition of contributions of GitHub users (year before collection). \\
\verb+users+ & Listing users (who can have several identities: email, GitHub, Gitlab) \\
\verb+watchers+ & Listing watchers (developers being notified of changes) of each repository \\
%\bottomrule
\hline

==> inputs/variables.tex <==
\newcommand\vartotalpackages{91,437}
\newcommand\varparsedpackages{74,829}
\newcommand\varclonedpackages{68,239}
\newcommand\varuniqueurls{51,657}
\newcommand\varuniquecloned{46,895}
\newcommand\varclonedgh{44,893}
\newcommand\varclonedgl{1,498}
\newcommand\varclonedall{46,895}
\newcommand\varcommitsnobots{5,656,407}
\newcommand\varbotsgh{219}
\newcommand\varghusers{58,329}
\newcommand\varglusers{450}
\newcommand\varnoghglusers{14,266}
\newcommand\vartotalemails{89,399}
\newcommand\varmatchingghglusers{87}
\newcommand\varclonedothergit{504}


\newcommand\varghtreposght{13,623}
\newcommand\varghtreposrust{16,069}
\newcommand\varghtcommitsght{1,299,414}
\newcommand\varghtcommitsrust{1,942,997}
\newcommand\varghtusersght{14,563}
\newcommand\varghtusersrust{21,989}



==> rust_scientific_data_accepted (1)/inputs/tables_description.tex <==
%\toprule
%\hline
\setlength\tabcolsep{2.5pt}
Table Name & Description\\
%\midrule
\hline
\verb+commit_comment_reactions+ & Individual emoji reactions to commit comments \\
\verb+commit_comments+ &  Comments to commits \\
\verb+commit_parents+ & Parenthood relationships between commits. Typically one per commit, can be 0 or more. \\
\verb+commit_repos+ & Repos to which commits belong. Min. one, can be several via forks. \\
\verb+commits+ & Listing metadata about specific commits \\
\verb+filtered_deps_package+ & Packages wich are filtered when appearing as a dependency to avoid cycles \\
\verb+filtered_deps_packageedges+ & Dependency edges between packages filtered to avoid cycles \\
\verb+filtered_deps_repo+ & Repositories wich are filtered when appearing as a dependency to avoid cycles \\
\verb+filtered_deps_repoedges+ & Edges directly discarded in the dependency graph \\
\verb+followers+ & Listing followers of GitHub accounts \\
\verb+forks+ & Listing forks declared on GitHub \\
\verb+identities+ & Listing each individual identity of the developers (email, GitHub account, Gitlab account) \\
\verb+identity_types+ & Listing of identitiy types (email, GitHub account, Gitlab account) \\
\verb+issue_comment_reactions+ & Individual emoji reactions to issue comments \\
\verb+issue_comments+ & Comments to issues \\
\verb+issue_labels+ & Individual labels of each issue \\
\verb+issue_reactions+ & Individual emoji reactions to each issue \\
\verb+issues+ & Listing of issues per repository \\
\verb+merged_identities+ & Keeping track of identities having been merged, for information purposes \\
\verb+merged_repositories+ & Repositories having been merged (after identifying renaming or typo in URL) \\
\verb+org_memberships+ & Membership of organization declared on GitHub for GitHub users. \\
\verb+organizations+ & Organizations or work groups as declared on GitHub \\
\verb+package_dependencies+ & Listing package dependencies (version to package with semver) \\
\verb+package_version_downloads+ & Listing daily downloads of package versions \\
\verb+package_versions+ & Listing versions of packages \\
\verb+packages+ & Listing packages \\
\verb+pullrequest_comment_reactions+ & Individual emoji reactions to each pull request \\
\verb+pullrequest_comments+ & Comments to each pull request \\
\verb+pullrequest_labels+ & Individual labels of each pull request \\
\verb+pullrequest_reactions+ & Individual emoji reactions to each pull request \\
\verb+pullrequests+ & Listing of pull requests per repository \\
\verb+repo_languages+ & Listing language composition of repositories (GitHub) \\
\verb+repositories+ & Listing repositories \\
\verb+sources+ & Listing data sources \\
\verb+sponsors_user+ & Listing sponsorships of developers \\
\verb+stars+ & Listing starring events of repositories \\
\verb+urls+ & Listing retrieved URLs, and their parsed equivalent \\
\verb+user_languages+ & Language composition of contributions of GitHub users (year before collection). \\
\verb+users+ & Listing users (who can have several identities: email, GitHub, Gitlab) \\
\verb+watchers+ & Listing watchers (developers being notified of changes) of each repository \\
%\bottomrule
\hline

==> rust_scientific_data_accepted (1)/inputs/variables.tex <==
\newcommand\vartotalpackages{91,437}
\newcommand\varparsedpackages{74,829}
\newcommand\varclonedpackages{68,239}
\newcommand\varuniqueurls{51,657}
\newcommand\varuniquecloned{46,895}
\newcommand\varclonedgh{44,893}
\newcommand\varclonedgl{1,498}
\newcommand\varclonedall{46,895}
\newcommand\varcommitsnobots{5,656,407}
\newcommand\varbotsgh{219}
\newcommand\varghusers{58,329}
\newcommand\varglusers{450}
\newcommand\varnoghglusers{14,266}
\newcommand\vartotalemails{89,399}
\newcommand\varmatchingghglusers{87}
\newcommand\varclonedothergit{504}


\newcommand\varghtreposght{13,623}
\newcommand\varghtreposrust{16,069}
\newcommand\varghtcommitsght{1,299,414}
\newcommand\varghtcommitsrust{1,942,997}
\newcommand\varghtusersght{14,563}
\newcommand\varghtusersrust{21,989}


